Contextualizing Meta-Learning via Learning to Decompose

Meta-learning has emerged as an efficient approach for constructing target models based on support sets. For example, the meta-learned embeddings enable the construction of target nearest-neighbor classifiers for specific tasks by pulling instances closer to their same-class neighbors. However, a single instance can be annotated from various latent attributes, making visually similar instances inside or across support sets have different labels and diverse relationships with others. Consequently, a uniform meta-learned strategy for inferring the target model from the support set fails to capture the instance-wise ambiguous similarity. To this end, we propose Learning to Decompose Network (LeadNet) to contextualize the meta-learned ``support-to-target'' strategy, leveraging the context of instances with one or mixed latent attributes in a support set. In particular, the comparison relationship between instances is decomposed w.r.t. multiple embedding spaces. LeadNet learns to automatically select the strategy associated with the right attribute via incorporating the change of comparison across contexts} with polysemous embeddings. We demonstrate the superiority of LeadNet in various applications, including exploring multiple views of confusing data, out-of-distribution recognition, and few-shot image classification.

==> info.tex <==

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/yehj.jpg}}]{Han-Jia Ye} received his Ph.D. degree in computer science from Nanjing University in 2019. He is currently an associate professor in the School of Artificial Intelligence at Nanjing University. His research focuses primarily on machine learning, with interests in representation learning, model reuse, and meta-learning. He has served as the Tutorial Co-Chair for SDM 2023 and the Doctoral Forum Co-Chair for SDM 2022. Additionally, he participates as a program committee member in conferences such as ICML, NeurIPS, ICLR.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/zhoudw.jpg}}]{Da-Wei Zhou}	is working towards the Ph.D. degree
	with the State Key Lab for Novel Software
	Technology, the Department of Computer
	Science~\& Technology in Nanjing University,
	China. His research interests lie primarily in machine
	learning and data mining. He is currently working on incremental learning. He serves as PC
	in leading conferences such as NeurIPS, ICLR, CVPR,
	ICCV, ECCV, etc.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/honglq.jpg}}]{Lanqing Hong} received her Bachelor's degree from Shanghai Jiao Tong University in 2014, and her PhD degree from the National University of Singapore in 2018. Her research interests include Computer Vision, Self-supervised Learning, Out-of-distribution Generalization, and Generative Models. She has published papers in top conferences, including CVPR, ICLR, NeurIPS, ICML, ICCV, ECCV, and others. She served as a Senior Program Committee member for IJCAI 2023 and has been a reviewer for TPAMI, ICML, NeurIPS, ICLR, CVPR, and others.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/lizg.jpg}}]{Zhenguo Li}	received the BS and MS degrees from the Department of Mathematics, Peking University, and the PhD degree from the Department of Information Engineering, Chinese University of Hong Kong. He is currently the director with AI Theory Lab, Huawei Noah’s Ark Lab. Before joining Huawei, he was an associate research scientist with the Department of Electrical Engineering, Columbia University. His research interests include machine learning and artificial intelligence.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/weixs.jpg}}]{Xiu-Shen Wei}is a Professor with the School of Computer Science and Engineering, Southeast University, China. He was a Program Chair for the workshops associated with ICCV, IJCAI, ACM Multimedia, etc. He has also served as an Area Chair or Senior Program Member at CVPR, AAAI, IJCAI, ICME, BMVC, a Guest Editor of Pattern Recognition Journal, and a Tutorial Chair for Asian Conference on Computer Vision (ACCV) 2022.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figures/zdc.jpg}}]{De-Chuan Zhan}
	received the Ph.D. degree in computer science, Nanjing University, China in 2010, then he became a faculty
	member in the Department of Computer Science
	and Technology at Nanjing University, China. He
	is currently a Professor at the School of Artificial Intelligence at Nanjing University. His research interests are mainly in machine learning, data mining, and mobile intelligence. He has published over 90 papers in leading international journal/conferences. He serves as an editorial board member of IDA and IJAPR, and serves as SPC/PC in leading conferences such as IJCAI, AAAI, ICML, NeurIPS, etc.
\end{IEEEbiography}



==> math_definition.tex <==
%%% load AMS-Latex Package
\usepackage{amssymb}
\usepackage{amsmath,amsfonts}
% \usepackage{amsthm}
\usepackage{amsopn}
\usepackage{bm} % bold symbol
\usepackage{multirow}
%\usepackage{threeparttable}
\usepackage{flushend}
\usepackage{tabularx}
%\usepackage{tablestyles}
% define vector and matrix symbols
\newcommand{\vct}[1]{\boldsymbol{#1}} % vector
\newcommand{\mat}[1]{\boldsymbol{#1}} % matrix
\newcommand{\cst}[1]{\mathsf{#1}}  % constant

%%%% Special math symbols
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\R}{\field{R}} % real domain
\newcommand{\C}{\field{C}} % complex domain
\newcommand{\F}{\field{F}} % functional domain
\newcommand{\I}{\field{I}} % functional domain
\newcommand{\T}{^{\textrm T}} % transpose


%% operator in linear algebra, functional analysis
\newcommand{\inner}[2]{#1\cdot #2}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\twonorm}[1]{\left\|#1\right\|_2^2}
\newcommand{\onenorm}[1]{\|#1\|_1}
\newcommand{\Map}[1]{\mathcal{#1}}  % operator in functions, maps such as M: domain1 --> domain 2

% operator in probability: expectation, covariance, 
\newcommand{\ProbOpr}[1]{\mathbb{#1}}
% independence
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\ind}[2]{{#1} \independent{#2}}
\newcommand{\cind}[3]{{#1} \independent{#2}\,|\,#3} % conditional independence
\newcommand{\expect}[2]{%
\ifthenelse{\equal{#2}{}}{\ProbOpr{E}_{#1}}
{\ifthenelse{\equal{#1}{}}{\ProbOpr{E}\left[#2\right]}{\ProbOpr{E}_{#1}\left[#2\right]}}} % Expectation: syntax: E{1}{2} = E_1[2], E{}{2}=E[2], E{1}{} = E_1
\newcommand{\var}[2]{%
\ifthenelse{\equal{#2}{}}{\ProbOpr{VAR}_{#1}}
{\ifthenelse{\equal{#1}{}}{\ProbOpr{VAR}\left[#2\right]}{\ProbOpr{VAR}_{#1}\left[#2\right]}}} % Expectation: syntax: V{1}{2} = V_1[2], V{}{2}=V[2], V{1}{} = V_1
\newcommand{\cndexp}[2]{\ProbOpr{E}\,[ #1\,|\,#2\,]}  % conditional expectation

% operator in optimization
\DeclareMathOperator{\argmax}{arg\,max}
\DeclareMathOperator{\argmin}{arg\,min}
\DeclareMathOperator{\softmax}{softmax}

% special functions
\newcommand{\trace}[1]{\operatornamewithlimits{tr}\left\{#1\right\}}
\newcommand{\diag}{\operatornamewithlimits{diag}}
\newcommand{\sign}{\operatornamewithlimits{sign}}
\newcommand{\const}{\operatornamewithlimits{const}}

% special display
\newcommand{\parde}[2]{\frac{\partial #1}{\partial  #2}}


% environment
% \newtheorem{thm}{Theorem}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{proposition}[theorem]{Proposition}

% shorthand
\newcommand{\vtheta}{\vct{\theta}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vx}{{\vct{x}}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{{\vct{z}}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vo}{{\vct{o}}}
\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vt}{\vct{t}}
%\newcommand{\vpsi}{\vct{\psi}}
% \newcommand{\vs}{\vct{s}}
\newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vzero}{\vct{0}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\ones}{\vct{1}}
\newcommand{\mU}{\mat{U}}
\newcommand{\mA}{\mat{A}}
\newcommand{\mB}{\mat{B}}
\newcommand{\mD}{\mat{D}}
\newcommand{\mW}{\mat{W}}
\newcommand{\mH}{\mat{H}}
\newcommand{\mS}{\mat{S}}
\newcommand{\mJ}{\mat{J}}
\newcommand{\mM}{\mat{M}}
\newcommand{\mT}{\mat{T}}
\newcommand{\mZ}{\mat{Z}}
\newcommand{\mO}{\mat{O}}
\newcommand{\mY}{\mat{Y}}
\newcommand{\mL}{\mat{L}}
\newcommand{\mI}{\mat{I}}
\newcommand{\mK}{\mat{K}}
\newcommand{\mSigma}{\mat{\Sigma}}
\newcommand{\mOmega}{\mat{\Omega}}
\newcommand{\cC}{\cst{C}}
\newcommand{\cM}{\cst{M}}
\newcommand{\cN}{\cst{N}}
\newcommand{\cQ}{\cst{Q}}
\newcommand{\cD}{\cst{D}}
\newcommand{\cL}{\cst{L}}
\newcommand{\cK}{\cst{K}}
\newcommand{\cH}{\cst{H}}
\newcommand{\cR}{\cst{R}}
\newcommand{\cU}{\cst{U}}
\newcommand{\cS}{\cst{S}}
\newcommand{\sQ}{\mathcal{Q}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sC}{\mathcal{C}}


% 
\newcommand{\nx}{\tilde{x}}
\newcommand{\vnx}{{\tilde{\vx}}}
\newcommand{\vnz}{{\tilde{\vz}}}
%\newcommand{\deltavx}{(\vnx-\vx)}
\newcommand{\deltavx}{\delta_\vx}
\newcommand{\vmx}{\bar{\vx}}
\newcommand{\vmz}{\bar{\vz}}
\newcommand{\sigmax}{\mSigma_{\vx}}
\newcommand{\sigmaz}{\mSigma_{\vz}}
\newcommand{\no}{\tilde{o}}
\newcommand{\vno}{{\tilde{\vo}}}
\newcommand{\nell}{\tilde{\ell}}
\newcommand{\jacob}{\mat{J}}
\newcommand{\hess}{\mat{H}}
\newcommand{\mloss}{\hat{\ell}}

%
\newcommand{\eat}[1]{}
\newcommand{\method}[1]{\textsc{#1}}
\newcommand{\task}[1]{\textbf{#1}}
\newcommand{\GDC}{\method{GDC}\xspace}
\newcommand{\SDN}{\method{SDN}\xspace}
\newcommand{\GSTD}{\method{GS3D}\xspace}
\newcommand{\vPIXOR}{\method{PIXOR$^\star$}\xspace}
\newcommand{\PIXOR}{\method{PIXOR}\xspace}
\newcommand{\PRCNN}{\method{P-RCNN}\xspace}
\newcommand{\SRCNN}{\method{S-RCNN}\xspace}
\newcommand{\PL}{\method{pseudo-LiDAR}\xspace}
\newcommand{\AVOD}{\method{AVOD}\xspace}
\newcommand{\Frustum}{\method{F-PointNet}\xspace}
\newcommand{\Mono}{\method{Mono3D}\xspace}
\newcommand{\DOP}{\method{3DOP}\xspace}
\newcommand{\DORN}{\method{DORN}\xspace}
\newcommand{\MLF}{\method{MLF}\xspace}
\newcommand{\MLFmono}{\method{MLF-mono}\xspace}
\newcommand{\MLFstereo}{\method{MLF-stereo}\xspace}

\newcommand{\APBEV}{AP$_\text{BEV}$\xspace}
\newcommand{\AP}{AP$_\text{3D}$\xspace}

\newcommand{\PSMNet}{\method{PSMNet}\xspace}
\newcommand{\PSMNetpd}{\method{PSMNet}\xspace}
\newcommand{\DispNet}{\method{DispNet}\xspace}
\newcommand{\DispNetS}{\method{DispNet-S}\xspace}
\newcommand{\DispNetC}{\method{DispNet-C}\xspace}
\newcommand{\SPSstereo}{\method{SPS-stereo}\xspace}
\newcommand{\PnP}{\method{PnP}\xspace}
